Diminished circadian and ultradian rhythms of human brain activity in pathological tissue in vivo

Chronobiological rhythms, such as the circadian rhythm, have long been linked to neurological disorders, but it is currently unknown how pathological processes affect the expression of biological rhythms in the brain. Here, we use the unique opportunity of long-term, continuous intracranially recorded EEG from 38 patients (totalling 6338 hours) to delineate circadian (daily) and ultradian (minute to hourly) rhythms in different brain regions. We show that functional circadian and ultradian rhythms are diminished in pathological tissue, independent of regional variations. We further demonstrate that these diminished rhythms are persistent in time, regardless of load or occurrence of pathological events. These findings provide evidence that brain pathology is functionally associated with persistently diminished chronobiological rhythms in vivo in humans, independent of regional variations or pathological events. Future work interacting with, and restoring, these modulatory chronobiological rhythms may allow for novel therapies.

==> suggest_reviewers.tex <==
"Maxime Baud" <maxime.baud@insel.ch>
"Felix Chan" <f.chan2@aston.ac.uk>
"Pip Karoly" <karoly.p@unimelb.edu.au>
"Skarke, Carsten" <cskarke@pennmedicine.upenn.edu>
"Sridevi Sarma" <ssarma2@jhu.edu>
"Sharon Chiang" <sharon.chiang@ucsf.edu>
"Ankit Khambhati" <Ankit.Khambhati@ucsf.edu>
"Adrià Tauste" <adria.tauste@upc.edu>
"Beth A Lopour" <blopour@uci.edu>
"Christian Meisel" <chr.meisel@charite.de>
"Mark Richardson" <mark.richardson@kcl.ac.uk>
"Andreas Schulze-Bonhage" <andreas.schulze-bonhage@uniklinik-freiburg.de>
"Hugh Piggins" <hugh.piggins@bristol.ac.uk>

